Architectural Complexity Measures of Recurrent Neural Networks

In this paper, we systematically analyze the connecting architectures of recurrent neural networks (RNNs). Our main contribution is twofold: first, we present a rigorous graph-theoretic framework describing the connecting architectures of RNNs in general. Second, we propose three architecture complexity measures of RNNs: (a) the recurrent depth, which captures the RNN's over-time nonlinear complexity, (b) the feedforward depth, which captures the local input-output nonlinearity (similar to the "depth" in feedforward neural networks (FNNs)), and (c) the recurrent skip coefficient which captures how rapidly the information propagates over time. We rigorously prove each measure's existence and computability. Our experimental results show that RNNs might benefit from larger recurrent depth and feedforward depth. We further demonstrate that increasing recurrent skip coefficient offers performance boosts on long term dependency problems.

==> 1recdepth.tex <==
\title{Architectural Complexity Measures of \\ Recurrent Neural Networks}

% The \author macro works with any number of authors. There are two
% commands used to separate the names and addresses of multiple
% authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to
% break the lines. Using \AND forces a line break at that point. So,
% if LaTeX puts 3 of 4 authors names on the first line, and the last
% on the second line, try using \AND instead of \And before the third
% author name.

\author{Saizheng Zhang$^{1,}$\thanks{Equal contribution.}, Yuhuai Wu$^{2,*}$, Tong Che$^4$, Zhouhan Lin$^1$, \\
\textbf{Roland Memisevic$^{1,5}$, Ruslan Salakhutdinov$^{3,5}$ and Yoshua Bengio$^{1,5}$}\\
$^1$MILA, Universit\'e de Montr\'eal, $^2$University of Toronto, $^3$Carnegie Mellon University,\\
$^4$Institut des Hautes \'Etudes Scientifiques, France, $^5$CIFAR\\
%\texttt{\{saizhenglisa, tongcheprivate, roland.umontreal, yoshua.bengio\}@gmail.com,} \\ \texttt{ywu@cs.toronto.edu, rsalakhu@cs.cmu.edu} \\
  %% examples of more authors
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \AND
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
}
\vspace{-25pt}
% \nipsfinalcopy is no longer used

\maketitle
\begin{abstract} 
In this paper, we systematically analyze the connecting architectures
of recurrent neural networks (RNNs). Our main contribution is twofold:
first, we present a rigorous graph-theoretic framework describing the
connecting architectures of RNNs in general.
Second, we propose three 
architecture complexity measures of RNNs: (a) the {\bf recurrent depth}, which
captures the RNN's over-time nonlinear complexity, (b)
the {\bf feedforward depth}, which captures the local input-output nonlinearity (similar
to the ``depth'' in feedforward neural networks (FNNs)), 
and (c) the {\bf recurrent skip coefficient}
which captures how rapidly the information
propagates over time. We rigorously prove each measure's existence and computability.
Our experimental results show that RNNs might benefit
from larger recurrent depth and feedforward depth.
We further demonstrate that increasing recurrent skip coefficient
offers performance boosts on long term dependency problems.
%as we improve the state-of-the-art for sequential MNIST dataset.
%as we found with an architecture that improves on the state of the art for $\tanh$ RNNs.
%LSTMs also benefit much
%from recurrent skip coefficients on the speed of convergence and test performance.


%Depth  is  a  conventional  complexity  measure  of  a  neural network.  Unlike feedforward neural networks (FNNs), where the notion of depth is well-defined, it is non-trivial to define a similar notion on Recurrent Neural networks (RNNs): even an non-stacked RNN have multiple layers when it is unfolded over time. In this paper, we firstly present a new framework for analyzing connections and depth in RNNs, by formally describing two graph representations of an general RNN architecture.  We then propose three crucial measures of complexity related to the notion of the depth in an RNN: the recurrent depth, the feedforward depth and the recurrent skip coefficient. The recurrent depth and the feedforward depth respectively captures the architectural complexity of an RNN in the long run and in the short run, whereas the recurrent skip coefficient captures how rapidly information propagates over time. It turns out that with larger recurrent depth and feedforward depth, the performance is usually better. Moreover, increasing recurrent skip coefficient also offers a performance boost on tasks dealing with long term dependency: our model with large recurrent skip coefficient achieves the state of art in the sequential MNIST task for simple RNNs.
\end{abstract}
\section{Introduction}
\vspace{-5pt}
\label{sec:intro}
Recurrent neural networks (RNNs) have been shown to achieve promising results 
%Recently there has been an increasing number of
%successes for various types of recurrent neural networks (RNNs)
on many difficult sequential learning problems \cite{graves2013generating,
bahdanau2014neural, sutskever2014sequence, nitish_video, kiros_skipthought}.
There is also much work attempting to
reveal the principles behind the challenges and successes of RNNs,
including optimization issues \cite{martens2011learning, pascanu2013difficulty}, gradient vanishing/exploding related problems
\cite{hochreiter1991untersuchungen,bengio1994learning},
 analysing/designing new RNN transition functional units
like LSTMs, GRUs and their variants \cite{hochreiter1997long,
greff2015lstm, cho2014learning, jozefowicz2015empirical}. 

This paper focuses on another important theoretical aspect of RNNs:
the connecting architecture. Ever since
\cite{schmidhuber1992learning, el1996hierarchical}
introduced  different forms of ``stacked RNNs'', researchers
have taken architecture design for granted and have paid less
attention to the exploration of other connecting architectures.
%Only a few researches has been done alone this direction: 
Some examples include
\cite{raiko2012deep, graves2013generating, hermans2013training}
who explored the use of skip connections;
%\cite{hermans2013training} who proposed the deep RNNs which are stacked RNNs with skip connections;
 \cite{pascanu2013construct} who pointed out the distinction of
 constructing a ``deep'' RNN from the view of the recurrent
paths and the view of the input-to-hidden and hidden-to-output maps.
However, they did not rigorously formalize the notion of
``depth'' and its implications in ``deep'' RNNs. 
Besides ``deep'' RNNs, there still remains a vastly
unexplored field of connecting architectures.
We argue that one barrier for
better understanding the architectural complexity
is the lack of a general definition of the connecting architecture. This forced previous researchers 
to mostly consider the simple cases while
neglecting other possible connecting variations. Another barrier is the lack
of quantitative measurements of the complexity of different RNN connecting
architectures: even the concept of ``depth'' is not clear
with current RNNs.


In this paper, we try to address these two barriers.
We first introduce a general formulation of RNN connecting architectures, using 
%We first introduce a general definition of connecting architectures, where we divide an 
%RNN into two basic ingredients:
a well-defined graph representation.
%representation of
%the connecting architecture, and a set of transition functions describing the computational process associated with each unit in the network.
Observing that the RNN undergoes multiple transformations not only feedforwardly
(from input to output within a time step) but also recurrently
(across multiple time steps),  we carry out a quantitative analysis of
the number of transformations in these two orthogonal directions,
which results in the definitions of \emph{recurrent depth}
and \emph{feedforward depth}.
These two depths can be viewed as general extensions of the work of 
\cite{pascanu2013construct}.
We also explore a quantity called the \emph{recurrent skip coefficient}
which measures how quickly information propagates over time. This quantity
is strongly related to vanishing/exploding gradient issues, and helps deal with long term dependency problems. 
Skip connections crossing different timescales have also been 
studied by 
%Related work along this line includes 
\cite{Lin-ieeetnn96, el1996hierarchical, sutskever2010temporal, koutnik2014clockwork}.
%in which they proposed connections crossing different timescales.
Instead of specific architecture design, we focus on analyzing
the graph-theoretic properties of recurrent skip coefficients, revealing the fundamental difference
between the regular skip connections and the ones which truly increase the recurrent skip coefficients. 
We rigorously prove each measure’s existence and computability under the general framework.


%Recurrent neural networks (RNNs)have recently become a popular
%model for modeling variable-length sequences. Due to its great success over a wide range of tasks, researchers have been studying and developing architectures for RNNs (cite), including the commonly used ``deep'' stacked RNNs (cite), clockwork RNN that has asynchronous units and etc..

%Despite its great empirical successes, there have not been many theoretical discussions on this model. The most obvious barrier for doing theoretical analysis is the lack of a general definition. Previous definitions only consider the most simplest form of an RNN, but it is not suited for other proposed variations. To cater for such needs, in section 2, we introduce a general definition of RNNs. Here, we propose to think of an RNN in terms of its two ingredients: a graph representation of the connecting architecture, and a set of transition functions that defines the computational process within each unit. Those two components can be almost arbitrarily complex, thus containing previously proposed variations of RNN as a special case.

%The proposed definition provides a general framework under which we can explore the architectural complexity of RNNs. One conventional characterization of the architectural complexity for feedforward models is the notion of the depth, which is usually understood as the total number of layers in the network. However, it is non-trivial to define the depth of an RNN: even an non-stacked RNN has multiple layers if it is unfolded over time, as suggested by \cite{Pascanu+et+al-ICLR2014}. Unlike FNNs, the RNN is a dynamic system that undergoes transformations not only feedforwardly (within a time step) but also recurrently (over time steps), which forms two series of orthogonal computations. This motivates us to define depth in these two different perspective, which results in the definitions of \emph{recurrent depth} and \emph{feedforward depth}. In addition, we also consider a quantity called \emph{recurrent skip coefficient} that naturally derived from studying the architecture of an RNN: a quantity that measures how quickly information propagates over time. This quantity is informative in the tasks that deal with long term dependency. In particular, previous experiments (cite) show that adding skip connections which enlarges recurrent skip coefficient gains a significant performance boost in those tasks. In-depth discussions of three measures constitute section 3.

We empirically evaluate models with
different recurrent/feedforward depths and  
recurrent skip coefficients on
various sequential modelling tasks.
%language modelling and sequential MNIST tasks.
We also show 
that our experimental results further validate 
the usefulness of the proposed definitions.
%We highlight Section \ref{sec:depth_nontrivial}
%and Section \ref{sec:skip_nontrivial} to the reader, where the significance of
%the proposed measures are demonstrated by
%analysing models which look quite similar but have quite different performances. 
 


\section{General Formulations of RNN Connecting Architectures}
\vspace{-5pt}
RNNs are learning machines that recursively compute new
states by applying transition functions to previous states and inputs.
Its connecting architecture
describes how information flows between different nodes.
%The connecting architecture is usually illustrated informally by an
%infinite directed acyclic graph, which in turn can be viewed as a finite directed
%cyclic graph that is unfolded through time. 
%Such informality typically limits one
%to consider simple connecting architectures as mentioned in Section \ref{sec:intro}.
%These two kinds of graphical representations are widely
%used in literatures \textcolor{red}{(TODO:CITE)},
%but they have never been formalized.
%Also, in addition to the the specific function designation like
%LSTMor GRU\cite{cho2014learning},
%the transition functions could be formed with larger freedoms .
%In this section, we first introduce a general definition of the connecting
%architecture and its underlying computation, followed by a general definition of an RNN.
%Commonly used transition functions include basic RNN functions (e.g. tanh, sigmoid), LSTM, GRU, and even randomly sampled transition functions built of some basic gating units (cite emprical structure).
%\subsection{The Connecting Architecture}
%\label{sec:connect_arch}
In this section, we formalize the concept of the connecting architecture by extending the traditional graph-based illustration 
to a more general definition with a \emph{finite directed multigraph} and its \emph{unfolded} version. 
Let us first define the notion of the 
\emph{RNN cyclic graph} $\mathcal{G}_c$ that can be viewed as a cyclic graphical representation of RNNs.
% TODO: to make the following understandable, I have added the stuff below to state right away what the integer labels
% will be used for, at least informally (outside of the formal definition, either just before
% or just after)
We attach ``weights'' to the edges in the cyclic graph $\mathcal{G}_c$ that represent time delay differences between the
source and destination node in the unfolded graph.
\begin{defn}
\label{def:cyc}
\emph{
Let $\mathcal{G}_c = (V_c, E_c)$ be a weighted directed multigraph
\footnote{A directed multigraph is a directed graph
that allows multiple directed edges connecting two nodes.},
in which $V_c = V_{\tmop{in}} \cup V_{\tmop{out}} \cup V_{\tmop{hid}}$ is a finite nonempty
set of nodes, $E_c \subset V_c \times V_c \times \mathbb{Z}$ is a finite set of directed edges.
%and $V_{\tmop{in}}, V_{\tmop{out}}, V_{\tmop{hid}}$ are not empty. 
Each $e =(u,v,\sigma) \in E_c$ denotes a directed weighted edge pointing from node $u$ to node $v$ with an integer weight $\sigma$. Each node $v \in V_c$ is \ labelled by an integer tuple $(i, p)$. $i \in \{ 0, 2, \cdots m-1 \}$ denotes the time index of the given node, where $m$ is the \textbf{period number} of the RNN, and $p
\in S$, where $S$ is a finite set of node labels.
We call the
weighted directed multigraph $\mathcal{G}_c = (V_c, E_c)$ an RNN cyclic graph, if
}
\emph{
(1) For every edge $e =(u,v,\sigma) \in E_c$, let $i_u$ and $i_v$ denote the time index of node $u$ and $v$, then $\sigma = i_v-i_u+k\cdot m$ for some $k \in \mathbb{Z}$.
}
\emph{
(2) There exists at least one directed cycle
\footnote{A directed cycle is a closed walk with no
repetitions of edges.}
in $\mathcal{G}_c$. 
}
\emph{
(3) For any closed walk $\omega$, the sum of all the $\sigma$ along $\omega$ is not zero.
}
%
%\emph{
%(4)  There are no incoming edges to nodes in $V_{\tmop{in}}$, and
%no outgoing edges from nodes in $V_{\tmop{out}}$. There are both incoming edges and outgoing edges for nodes in $V_{\tmop{hid}}$.
%}
\end{defn}

%\vspace{-5pt}
%TODO Not Clear!!!
Condition (1) assures that we can get a periodic graph (repeating pattern) when unfolding the RNN through time.
Condition (2) excludes feedforward neural networks in the definition by forcing to have at least one cycle
in the cyclic graph.
Condition (3) simply avoids cycles after unfolding.
The cyclic representation can be seen as a time folded representation of RNNs,
as shown in Figure \ref{fig:basic}(a). Given an RNN cyclic graph $\mathcal{G}_c$, we unfold $\mathcal{G}_c$ over time $t\in \mathbb{Z}$
by the following procedure:

\begin{defn}[\bf Unfolding]
\label{def:un}
\emph{
Given an RNN cyclic graph \ $\mathcal{G}_c = (V_c, E_c, \sigma)$, we
define a new infinite set of nodes $V_{un} = \{ (i + k m, p) | (i, p) \in V, k
\in \mathbb{Z} \} \nobracket$. The new set of edges $E_{un} \in V_{un} \times
V_{un}$ is constructed as follows: \ $((t, p), (t', p')) \in E_{un}$ if and
only if there is an edge $e = ((i, p), (i', p'), \sigma) \in E$ such that $t' -
t = \sigma$, and $t \equiv i (\tmop{mod}
m)$. The new directed graph $\mathcal{G}_{\tmop{un}} = (V_{un}, E_{un})$ is called the unfolding of $\mathcal{G}_c$. Any infinite directed graph that can be constructed from an RNN cyclic graph through unfolding is called an RNN unfolded graph.
}
\end{defn}

\begin{lemma}
\label{prop:dag}
\emph{
The unfolding $\mathcal{G}_{\tmop{un}}$ of
any RNN cyclic graph $\mathcal{G}_c$ is a directed acyclic graph (DAG).
}
\end{lemma}

%\begin{exmp}
%\label{exp:rnndef}
Figure \ref{fig:basic}(a) shows an example of two graph representations $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$ of a given RNN. 
Consider the edge from node $(1,7)$ going to node $(0,3)$ in $\mathcal{G}_c$. The fact that it has weight 1 indicates that the corresponding edge in $\mathcal{G}_{\tmop{un}}$ travels one time step, $((t+1,7),(t+2,3))$. Note that node $(0,3)$ also has a loop with weight 2. This loop corresponds to the edge $((t,3),(t+2,3))$. 
%\end{exmp}
The two kinds of graph representations we presented above have a one-to-one correspondence.
 Also, any graph structure $\theta$ on $\mathcal{G}_{\tmop{un}}$ %such as node, edge or subgraph
 is naturally mapped into a graph structure $\bar{\theta}$ on $\mathcal{G}_c$. 
%(In topology, this mapping is called a covering map).  
 Given an edge tuple $\bar{e}=(u,v,\sigma)$ in $\mathcal{G}_c$, $\sigma$ stands for the number of time steps crossed by $\bar{e}$'s covering edges in $E_{un}$, i.e., for every corresponding edge $e\in \mathcal{G}_{\tmop{un}}$, $e$ must start from some time index $t$ to $t+\sigma$.
Hence $\sigma$ corresponds to the ``time delay'' associated with $e$. 
In addition, the \emph{period number}
$m$ in Definition \ref{def:cyc}
can be interpreted as the time length
of the entire non-repeated recurrent structure
in its unfolded RNN graph $\mathcal{G}_{\tmop{un}}$.
%Strictly speaking, 
%$m$ has the following properties in $\mathcal{G}_{\tmop{un}}$:
%$\forall k \in \mathbb{Z}$,
%if $\exists v = (t, p) \in V_{un}$,
%then $\exists v' = (t + km, p) \in V_{un}$;
%if $\exists e = ((t, p), (t', p')) \in E_{un}$,
%then $\exists e' = ((t+km, p), (t'+km, p')) \in E_{un}$.	
In other words, shifting the $\mathcal{G}_{\tmop{un}}$
through time by $km$ time steps will result in a 
DAG which is identical to $\mathcal{G}_{\tmop{un}}$,
and $m$ is the smallest number that has such property for $\mathcal{G}_{\tmop{un}}$.
Most traditional RNNs have $m = 1$, while some special
structures like {\em hierarchical} or {\em clockwork RNN}~\citep{el1996hierarchical, koutnik2014clockwork}
have $m>1$.
For example, Figure \ref{fig:basic}(a)
%from the unfolded graph representation $\mathcal{G}_{\tmop{un}}$, we can easily  
shows that the period number of this specific RNN is 2. 
%It is clear that if there exists 
%a directed cycle $\vartheta$ in $\mathcal{G}_c$, and
%the sum of $\sigma$
%along $\vartheta$ is positive (or negative),
%then there is a path which is the pre-image of $\vartheta$ in $\mathcal{G}_{\tmop{un}}$
%whose length (summing the edge $\sigma$'s) approaches $+\infty$ (or $-\infty$).
%This fact naturally induces the general definition of 
%unidirectionality and bidirectionality of RNNs as follows:
%\begin{defn}
%\emph{
%An RNN is called unidirectional if its cyclic
%graph representation $\mathcal{G}_c$ has the
%property that the sums of $\sigma$ along all the
%directed cycles $\vartheta$ in $\mathcal{G}_c$
%share the same sign, i.e., either all positive
%or all negative. An RNN is called bidirectional
%if it is not unidirectional.
%}
%\end{defn}

\begin{figure*}[t]
\includegraphics[width=\textwidth]{./figures/allexample_graph.pdf}
\vspace{-15pt}
\caption{\small (a) An example of an RNN's $\mathcal{G}_c$
and $\mathcal{G}_{\tmop{un}}$. $V_{\tmop{in}}$ is denoted
by square, $V_{\tmop{hid}}$ is denoted by circle and 
$V_{\tmop{out}}$ is denoted by diamond. In $\mathcal{G}_c$,
the number on each edge is its corresponding $\sigma$. The longest path is colored in red. The longest input-output path 
is colored in yellow and the shortest path is colored blue. The value of three measures are $d_r = \frac{3}{2}$, $d_f = \frac{7}{2}$ and $s = 2$. (b) 5 more examples. (1) and (2) have
$d_r = 2, \frac{3}{2}$, (3) has $d_f = 5$, (4) and (5) has $s = 2, \frac{3}{2}$.
}
\label{fig:basic}
\vspace{-15pt}
\end{figure*}
 The connecting architecture  describes how information flows 
 among RNN units. Assume $\bar{v} \in V_c$ is a node in $\mathcal{G}_c$, let $\mathrm{In}(\bar{v})$ denotes the set of incoming nodes of $\bar{v}$, $\mathrm{In}(\bar{v}) = \{\bar{u} | (\bar{u}, \bar{v}) \in E_{c}\}$. In the forward pass of the RNN, the transition function $F_{\bar{v}}$ takes outputs of nodes $\mathrm{In}(\bar{v})$ as inputs and computes a new output. For example, vanilla RNNs units with different activation functions, LSTMs and GRUs can all be viewed as units with specific transition functions. 
%The connecting architecture in Sec.~\ref{sec:connect_arch} describes how information flows 
%among RNN units. Assume $v\in V_c$ is a node in $\mathcal{G}_c$, let $\mathrm{In}(v)$ denotes the set of parents of $v$, $\mathrm{In}(v) = \{u | (u, v) \in E_{c}\}$. The transition function $F_v$ takes outputs of nodes $\mathrm{In}(v)$ as inputs and computes a new output. For example, vanilla RNNs can have different activation functions. More complex recurrent units,
%such as LSTMs~\citep{hochreiter1997long} and GRUs~\citep{cho2014learning},
%can also be viewed as transition functions. 
We now give the general definition of an RNN:
 \begin{defn}
 \em
 An RNN is a tuple $ (\mathcal{G}_{c},\mathcal{G}_{\tmop{un}}, \{F_{\bar{v}}\}_{\bar{v}\in V_{c}})$, 
 in which $\mathcal{G}_{\tmop{un}} = (V_{un}, E_{un})$ is the unfolding of RNN cyclic graph $\mathcal{G}_c$, and $\{F_{\bar{v}}\}_{\bar{v}\in V_{c}}$ is the set of transition functions. In the forward pass, for each hidden and output node $v \in V_{un}$, the transition function $F_{\bar{v}}$ takes all incoming nodes of $v$ as the input to compute the output. 
 \end{defn}
  An RNN is \emph{homogeneous} if all the hidden nodes share the same form of the transition function.% (but with perhaps different weight parameters).

%This is particularly interesting for the analysis of RNNs from the architectural point of view, where the nodes and edges in the graph are assumed to share the same functional meaning. 
%Our following work is also based on this assumption.
%It can be shown that with a more general definition, vanilla RNN, LSTM and GRU are homogeneous RNNs. For a more detailed analysis, see Appendix \ref{sec:LSTM}.
\section{Measures of Architectural Complexity}
%In this section we present our definitions of three architectural measures of RNNs.
%The connecting architecture and the transition functions of an RNN separately determines its complexity globally and locally. However, it is often difficult to obtain a quantitative measure from the perspective of transition functions. Instead, we focus at the architectural aspect of the complexity in this work, where our reasoning mostly rely on the graph-theoretic properties of RNNs. That being said, the complexity of transition functions is equally important, and additional analysis for future work is necessary to better understand the complexity of RNNs as a whole.
\vspace{-5pt}
In this section, we develop different measures of RNNs' architectural complexity, focusing mostly on the graph-theoretic properties of RNNs.
To analyze an RNN solely from its architectural aspect, we make the mild assumption that the RNN is homogeneous. 
We further assume the RNN to be unidirectional. For a bidirectional RNN, it is more natural to measure the complexities of its unidirectional components.
\vspace{-5pt}
\subsection{Recurrent Depth}
\vspace{-5pt}
Unlike feedforward models where computations are done within one time frame, RNNs map inputs to outputs over multiple time steps. In some sense, an RNN undergoes transformations along both feedforward and recurrent dimensions. This fact suggests that we should investigate its architectural complexity from these two different perspectives. We first consider the recurrent perspective.

The conventional definition of depth is the \emph{maximum} number of nonlinear transformations from inputs to outputs.
%~\citep{Bengio-2009-book}. 
Observe that a directed path in an unfolded graph representation $G_{un}$ corresponds to a sequence of nonlinear transformations. Given an unfolded RNN graph $G_{un}$, $\forall i,n \in \mathbb{Z}$, let $\mathfrak{D}_i(n)$ be
the length of the \emph{longest} path
from any node at starting time $i$ to any node at time $i+n$.
From the recurrent perspective, it is natural to investigate how $\mathfrak{D}_i(n)$ changes over time. Generally speaking, $\mathfrak{D}_i(n)$ increases as $n$ increases for all $i$. Such
increase is caused by the recurrent structure of the RNN
which keeps adding new nonlinearities over time. 
Since $\mathfrak{D}_i(n)$ approaches $\infty$ as $n$ approaches $\infty$,\footnote{Without loss of generality, we assume the unidirectional RNN approaches positive infinity.} to measure the complexity of $\mathfrak{D}_i(n)$, we consider its asymptotic behaviour, i.e., the limit of $\frac{\mathfrak{D}_i(n)}{n}$ as $n\to \infty$. Under a mild assumption, this limit exists.
%To perform a practical calculation of this limit, 
%the next theorem relies on $\mathcal{G}_{\tmop{un}}$'s cyclic counterpart $\mathcal{G}_{c}$, where the computation is much easier:
The following theorem prove such limit's computability and well-definedness: %relies on $\mathcal{G}_{\tmop{un}}$'s cyclic counterpart $\mathcal{G}_{c}$, where the computation is much easier:
\begin{thm}[\bf Recurrent Depth]
\label{thm:main-main}
%\vspace{-5pt}
Given an RNN and its two graph representation $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$, we denote $C (\mathcal{G}_c)$ to be the set of directed
  cycles in $\mathcal{G}_c$. For $\vartheta$ $\in C (\mathcal{G}_c)$, let  $l
  (\vartheta)$ denote the length of $\vartheta$ and $\sigma_s (\vartheta)$ denote the sum of edge weights
  $\sigma$ along $\vartheta$. Under a mild assumption\footnote{See a full treatment of the limit in general cases in Theorem \ref{thm:main} and Proposition \ref{prop:assump} in Appendix.},
  \begin{equation}
        \label{eqn:main1}
        d_r = \lim_{n \rightarrow +\infty}\frac{\mathfrak{D}_i(n)}{n} = \max_{\vartheta \in C (\mathcal{G}_c)} \frac{l (\vartheta)}{
       \sigma_s (\vartheta)}.
    \end{equation}
%Thus, $d_r$ is a positive rational number.
\end{thm} 
\vspace{-5pt}
More intuitively, $d_r$ is a measure of the average maximum number of nonlinear transformations per time step as $n$ gets large. Thus, we call it \emph{recurrent depth}:
\begin{defn}[\textbf{Recurrent Depth}]
%(\textbf{recurrent depth})
\emph{
Given an RNN and its two graph representations $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$,
we call $d_r$, defined in Eq.(\ref{eqn:main1}), the recurrent depth of the RNN.}
%\vspace{-10pt}
\end{defn}
%Given recurrent depth $d_r(\mathcal{E})$,
%the maiximal nonlinear dependencies from nodes at $t$ to the
%nodes at $t+n$ equals to $nd_r(\mathcal{E}) + c_n$ which
%is roughly $nd_r(\mathcal{E})$, and $c_n$ is some bounded constant depend on $n$.
%\begin{exmp}
%\label{exp:recdepth}

In Figure \ref{fig:basic}(a), one can easily verify that $\mathfrak{D}_t(1)=5$, $\mathfrak{D}_t(2)=6$, $\mathfrak{D}_t(3)=8$, $\mathfrak{D}_t(4)=9$ $\dots$ Thus $\frac{\mathfrak{D}_t(1)}{1} = 5$, $\frac{\mathfrak{D}_t(2)}{2} = 3$, $\frac{\mathfrak{D}_t(3)}{3} = \frac{8}{3}$, $\frac{\mathfrak{D}_t(4)}{4} = \frac{9}{4}$ $\dots$., which eventually converges to $\frac{3}{2}$ as $n \to \infty$.
As $n$ increases, most parts of the longest path coincides with the path colored in red. As a result, $d_r$ coincides with the number of nodes the red path goes through per time step. Similarly in $\mathcal{G}_c$, observe that the red cycle achieves the maximum ($\frac{3}{2}$) in Eq.(\ref{eqn:main1}). Usually, one can directly calculate $d_r$ from $\mathcal{G}_{\tmop{un}}$. 
%We introduce the computation in $\mathcal{G}_c$ for general purposes. 
%\vspace{-5pt}
%\end{exmp}
It is easy to verify that \emph{simple RNNs} and \emph{stacked RNNs} share the same recurrent depth which is equal to 1. This reveals the fact that their nonlinearities increase at the same rate, which suggests that 
they will behave similarly in the long run. This fact is often neglected, since one would 
typically consider the number of layers as a measure of depth, and think of stacked RNNs as ``deep'' and simple RNNs as ``shallow'', even though their discrepancies are not due to 
recurrent depth (which regards time) but due to feedforward depth, defined next.
\vspace{-5pt}
\subsection{Feedforward Depth}
\vspace{-5pt}
Recurrent depth does not fully characterize the nature of nonlinearity of an RNN. 
As previous work suggests \citep{sutskever2014sequence}, stacked
RNNs do outperform shallow ones with the same hidden size on problems where a more immediate
input and output process is modeled. This is not surprising, since the growth rate of $\mathfrak{D}_i(n)$ only captures the number of nonlinear transformations in the time direction, not in the feedforward direction.
The perspective of feedforward computation puts more emphasis on the specific paths connecting inputs to outputs. Given an RNN unfolded graph $G_{un}$, let $\mathfrak{D}^*_i(n)$ be the length of the longest path from any input node at time step~$i$ to any output node at time step $i+n$. Clearly, when $n$ is small, the recurrent depth cannot serve as a good description for $\mathfrak{D}^*_i(n)$. In fact. it heavily depends on another quantity which we call \emph{feedforward depth}. The following proposition guarantees
the existence of such a quantity and demonstrates the role of both measures in quantifying the nonlinearity of an RNN. 
%As experiements suggests, stacked RNNs do outperform simple ones with the same dimension of hidden space.
%While recurrent depth captures the complexity of an RNN in the long run, we should also investigate the short-run complexity: the number of functional transformations from an input to its \emph{closest} output.

%\begin{equation}
%{l_{t,n}^{{\max}^{*}}} = \underset{\substack{ \text{$\xi_{v,v'}^k \in \xi_{v,v'}$, $v =(t,0)$ }
%\\\text{  $v' =(t+n,r)$}}
%}{\operatorname{max}} \ 
%l(\xi_{v,v'}^k)
%\end{equation}

\begin{proposition}[\textbf{Input-Output Length Least Upper Bound}]
\label{prop:sup}
\em
Given an RNN with recurrent depth $d_r$, we denote 
$d_f = \sup_{i,n \in \mathbb{Z}}{\mathfrak{D}^*_i(n)} - n\cdot d_r$,
the supremum $d_f$ exists and thus we have the following upper bound for $\mathfrak{D}^*_i(n)$:
\vspace{-3pt}
\begin{equation*}
\mathfrak{D}^*_i(n)  \leq n\cdot d_r +d_f.
\end{equation*}
\end{proposition}
\vspace{-3pt}
The above upper bound explicitly shows the interplay between recurrent depth and feedforward depth: when $n$ is small, $\mathfrak{D}^*_i(n)$ is largely bounded by $d_f$; when $n$ is large, $d_r$ captures the nature of the bound ($\approx{n\cdot d_r}$). These two measures are equally important, as they separately capture the maximum number of nonlinear transformations of an RNN in the long run and in the short run. 

\begin{defn}
(\textbf{Feedforward Depth})\emph{
Given an RNN with recurrent depth $d_r$ and its two graph representations $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$, we call $d_f$, defined in Proposition~\ref{prop:sup}, the feedforward depth\footnote{Conventionally, an architecture with depth 1 is a three-layer architecture containing one hidden layer. But in our definition, since it goes through two transformations, we count the depth as 2 instead of 1. This should be particularly noted with the concept of feedforward depth, which can be thought as the conventional depth plus 1.} of the RNN.}
\end{defn}
\vspace{-7pt}
%To calculate $d_f$ in practice, we introduce the following theorem:
The following theorem proves $d_f$'s computability:
\begin{thm}[\textbf{Feedforward Depth}]
%\vspace{-5pt}
\label{thm:feed}
Given an RNN and its two graph representations $\mathcal{G}_{\tmop{un}}$ and
  $\mathcal{G}_c$, we denote $\xi (\mathcal{G}_c)$ the set of directed paths 
  that start at an input node and end at an output node in $\mathcal{G}_c$.
  For $\gamma \in \xi(\mathcal{G}_c)$, denote $l (\gamma)$ the length and
  $\sigma_s (\gamma)$ the sum of $\sigma$ along $\gamma$. Then we have:
  \begin{equation*}
      d_f = \sup_{i, n \in \mathbb{Z}} \mathfrak{D}_i^{\ast} (n) - n \cdot d_r
     = \max_{\gamma \in \xi (\mathcal{G}_c)} l (\gamma) - \sigma_s (\gamma)
     \cdot d_r,
  \end{equation*}
where $m$ is the period number and $d_r$ is the recurrent depth of the RNN. 
%Thus, $d_f$ is a postive rational number.
\end{thm}
%\begin{exmp}
%\label{exp:feeddepth}
For example, in Figure \ref{fig:basic}(a), one can easily verify that
$d_f=\mathfrak{D}^*_t(0)=3$. Most commonly, $d_f$ is the same as 
$ \mathfrak{D}^*_t(0)$, i.e., the maximum length from an input to its
current output. 
%\vspace{-5pt}
%\end{exmp}
\vspace{-2pt}
\subsection{Recurrent Skip Coefficient}
\vspace{-5pt}
Depth provides a measure of the complexity of the model.
But such a measure is not sufficient to characterize behavior on long-term dependency
tasks. In particular, since models with large recurrent depths have more nonlinearities through time, gradients can explode or vanish more easily. 
On the other hand, it is known 
%previous researches (see Introduction)
%empirically show 
that adding skip connections across multiple time steps
may help improve the performance on long-term dependency problems 
\cite{Lin-ieeetnn96, sutskever2010temporal}.
To measure such a ``skipping'' effect, we should instead pay attention to the 
length of the {\em shortest path} from time $i$ to time $i+n$. 
In $G_{un}$, $\forall i,n \in \mathbb{Z}$,
let $\mathfrak{d}_i(n)$ be the length of the shortest path.  
%be the length of the shortest path between time $i$ and time $i+n$. 
Similar to the recurrent depth, we consider the growth rate of $\mathfrak{d}_i(n)$.

\begin{thm}[\textbf{Recurrent Skip Coefficient}]
%\vspace{-5pt}
\label{thm:rsc}
Given an RNN and its two graph representations $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$, under mild assumptions\footnote{See Proposition \ref{prop:assump2} in Appendix.}
\vspace{-7pt}
\begin{equation}
\label{eqn:rsc}
j = \lim_{n \rightarrow +\infty}\frac{\mathfrak{d}_i(n)}{n} = \min_{\vartheta \in C (\mathcal{G}_c)} \frac{l (\vartheta)}{
       \sigma_s (\vartheta)}. 
\end{equation}
%Thus, $j$ is a positive rational number.
\end{thm}
\vspace{-5pt}
Since it is often the case that $j$ is smaller or equal to 1, it is more intuitive to consider its reciprocal.
\begin{defn}(\textbf{Recurrent Skip Coefficient})\footnote{One would find this definition very similar to the definition of the recurrent depth. Therefore, we refer readers to examples in Figure \ref{fig:basic} for some illustrations.}.
\emph{
Given an RNN and corresponding $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$, we define $s= \frac{1}{j}$, whose reciprocal is defined in Eq.(\ref{eqn:rsc}), as the recurrent skip coefficient of the RNN.}
%\vspace{-10pt}
\end{defn}
\vspace{-7pt}
With a larger recurrent skip coefficient, the number of transformations per time step is smaller. As a result, the nodes in the RNN are more capable of ``skipping'' across the network, allowing unimpeded information flow across multiple time steps, thus alleviating the problem of
learning long term dependencies. In particular, such effect is more prominent in the long run, due to the network's recurrent structure. 
Also note that not all types of skip connections can increase the recurrent skip coefficient. We will consider specific examples in our experimental results section.

%Given $\mathcal{G}_{\tmop{un}}$, let $\mathfrak{d}^*_i(n)$ be the length of the shortest paths from input nodes at time step $i$ to output nodes at time step $i+n$.

%\begin{thm}[(\textbf{Input-Output Length Greatest Lower Bound})]
%Given an RNN with recurrent depth $d_r$, we denote 
%\begin{equation}
%s^f = \inf_{i,n \in \mathbb{Z}}{\mathfrak{d}^*_i(n)} - n\cdot s^r
%\end{equation}
%The infimum $s^f$ exists and thus we have the following greatest lower bound for $\mathfrak{d}^*_i(n)$
%\begin{equation}
%\mathfrak{d}^*_i(n)  \geq n\cdot s^r +s^f
%\end{equation}
%\end{thm}

%To calculate $s^f$, we introduce the following theorem:
%\begin{thm}[\textbf{Main Theorem(Part II)}]
%\vspace{-5pt}
%\label{thm:recdepth}
%Given an RNN and its two graph representations $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$, 
%\begin{equation}
%\label{eq:ffsha}
%s^f = \inf_{i,n \in \mathbb{Z}}{\mathfrak{d}^*_i(n)} - n\cdot s^r = %\min_{\xi \in \xi(\mathcal{G}_c)}\: l(\xi)-\sigma_s(\xi)m\cdot s^r,
%\end{equation}
%where $m$, $s^r$ are the period number and the recurrent recurrent skip coefficient of the RNN. Thus, $s^f$ is a positive rational number.
%\end{thm}

%\begin{defn}
%(\textbf{Feedforward Shallowness})\emph{
%Given an RNN with the recurrent shallowness $s^r$ and its two graph representations $\mathcal{G}_{\tmop{un}}$ and $\mathcal{G}_c$, we call $s^f$ defined in Eq.(\ref{eq:ffsha}) the feedforward shallowness of the RNN.}
%\end{defn}
\vspace{-5pt}
\section{Experiments and Results}
\vspace{-5pt}
In this section we conduct a series of experiments to investigate the following
questions: (1) Is recurrent depth a trivial measure? (2) Can increasing depth yield performance improvements?
(3) Can increasing the recurrent skip coefficient improve the performance on long term dependency tasks? (4)
Does the recurrent skip coefficient suggest something more compared to simply adding skip
connections? 
We show our evaluations on both $\tanh$ RNNs and LSTMs.
%We first show evaluations on RNNs with
%\textit{tanh} nonlinearities, and then present similar results for LSTMs. 
%The results provide
%evidence for a negative answer for (1) and positive answers for (2),(3) and (4).

%Experiments in this section are conducted to validate the following
%five claims: (1) Recurrent depth measures complexity in a 
%non-trivial way. (2) Increasing depths can yield performance improvements. 
%(3) Increasing feedforward depth does not help on long
%term dependency tasks. (4) Increasing the recurrent skip coefficient
%largely improves the performance on long term dependency tasks. (5)
%Increasing recurrent skip coefficient is not as simple as adding skip
%connections. We first show all the evaluations on RNN with
%\textit{tanh},
%and then present similar results for LSTMs.

\vspace{-5pt}
\subsection{Tasks and Training Settings}
\vspace{-5pt}

\textbf{PennTreebank dataset}:
We evaluate our models on character level language modelling
using the PennTreebank dataset \cite{marcus1993building}. It contains 5059k characters
for training, 396k for validation and 446k for test, and has
a alphabet size of 50.
We set each training sequence to have the length of 50.
Quality of fit is evaluated by the bits-per-character (BPC) metric,
which is $\log_2$ of perplexity.

\textbf{text8 dataset}: Another dataset used for character level language modelling
is the text8 dataset\footnote{http://mattmahoney.net/dc/textdata.},
which contains $100M$ characters from Wikipedia 
with an alphabet size of 27. 
%letters \textit{a-z} and a space symbol.
We follow the setting from \cite{mikolov2012subword} and 
each training sequence has length of 180.
%: $90M$ for training, $5M$ for validation % TODO cite
%and the remaining $5M$ for test. We also divide the training set 
%into non-overlapping sequences, each of length $180$.

\textbf{adding problem}:
The adding problem (and the following copying memory problem) was 
introduced in \cite{hochreiter1997long}.
For the adding problem, 
each input has two sequences with length of $T$ where the first sequence are numbers sampled from
uniform[0, 1] and the second sequence are all zeros except two elements which
indicates the position of the two elements in the first sequence that should be
summed together. The output is the sum.
We follow the most recent results and experimental settings in \cite{arjovsky2015unitary} (same for copying memory).

\textbf{copying memory problem}:
Each input sequence has length of
$T + 20$, where the first $10$ values are random integers between $1$ to $8$.
The model should remember them after $T$ steps.
The rest of the sequence are all zeros, except for the last 11 entries in the sequence, which 
starts with $9$
as a marker indicating that the model should 
begin to output its memorized values. The model is expected to give
zero outputs at every time step except the last 10 entries, where it should
generate (copy) the $10$ values in the same order as it has seen at the beginning of the 
sequence.
The goal is to minimize the average cross entropy of category predictions at
each time step.

%\subsubsection{Sequenial MNIST}
\textbf{sequential MNIST dataset}:
%We also evaluate our models with a modified version of the MNIST dataset. 
Each MNIST image data is reshaped into a $784\times1$ sequence,
turning the digit classification task into a sequence classification one
with long-term dependencies~\citep{le2015simple,arjovsky2015unitary}.
%The model has access to $1$ pixel per time step and
%predicts the class label at the end.
A slight modification of the dataset is to permute
the image sequences by a fixed random order beforehand
(permuted MNIST).
%Since spatially local dependencies are no longer local
%(in the sequence), this task may be harder in terms of modelling long-term dependencies.
Results in \cite{le2015simple} have shown that both \textit{tanh} RNNs and LSTMs  % TODO cite
did not achieve satisfying performance, which also highlights the 
difficulty of this task. % for these two architectures.

%\subsection{Training Settings}
For all of our experiments  
we use \textit{Adam}~\citep{kingma2014adam} for optimization, and conduct 
a grid search
on the learning rate in $\{10^{-2}, 10^{-3},10^{-4},10^{-5}\}$.
For $\tanh$ RNNs, 
the parameters are initialized with samples from a uniform distribution.
% which limits are selected by grid search on
%range $\{10^{-1}, 10^{-2},10^{-3}\}$. 
For LSTM networks we adopt a similar initialization scheme, while
the forget gate biases are chosen by the grid search on $\{-5, -3, -1, 0, 1, 3, 5\}$.
We employ early stopping and the batch size was set to $50$.
\vspace{-8pt}
\subsection{\bf Recurrent Depth is Non-trivial}
\vspace{-5pt}
\label{sec:depth_nontrivial}
To investigate the first question, we compare 4 similar connecting architectures: 
1-layer (shallow) ``$sh$'', 2-layers stacked ``$st$'',
2-layers stacked with an extra bottom-up connection ``$bu$'', and
2-layers stacked with an extra top-down connection ``$td$'',
as shown in Figure~\ref{fig:depth_graph}(a), left panel. 
%compare to previous results reported in~\cite{pascanu2012understanding, mikolov2012subword}
%and we evaluate $\tanh$ RNNs (512 units for ``$sh$'', same size as \cite{pascanu2012understanding})
%and LSTMs (LSTMs-large with 1024 units for ``$sh$'' has the same size
%as \cite{mikolov2012subword}) using the four architectures above.
%\textit{sh} has a layer size of $512$, while the rest of the networks 
%have a layer size of $256$, making the number of hidden parameters
%in each architecture remain roughly the same.
%(denoted as ``P-$sh$''), since they used the 
%same model architecture as the one specified by our $sh$.  
Although the four architectures look quite similar, they have 
different recurrent depths: \textit{sh}, \textit{st} and \textit{bu} have
$d_r = 1$, while \textit{td} has $d_r = 2$. Note that the specific 
construction of the extra nonlinear transformations in 
\textit{td} is not conventional.
Instead of simply adding intermediate layers in hidden-to-hidden
connection, as reported in~\cite{pascanu2013construct}, more nonlinearities are gained by a 
recurrent flow from the first layer to the second layer and then back to the first layer 
at each time step (see the red path in Figure~\ref{fig:depth_graph}a, left panel).

We first evaluate our architectures using $\tanh$ RNN on PennTreebank,
where \textit{sh} has hidden-layer size of $1600$.
%(model size comparable to ),
Next, we  evaluate four different models for text8 which are $\tanh$ RNN-small,
$\tanh$ RNN-large, LSTM-small, LSTM large, where the model's \textit{sh} architecture
has hidden-layer size of 512, 2048, 512, 1024 respectively. 
Given the architecture of the \textit{sh} model, 
we set the remaining three architectures to have the same number of parameters.
Table \ref{tb:butd}, left panel, shows that the \textit{td} architecture outperforms all the other 
architectures for all the different models.
Specifically, 
\textit{td} in $\tanh$ RNN
achieves a test BPC of 1.49 on PennTreebank, which is comparable to  
the BPC of 1.48 reported in~\cite{krueger2015regularizing} using stabilization techniques.
Similar improvements are shown for LSTMs, where
\textit{td} architecture in LSTM-large achieves BPC of 1.49 on text8, outperforming 
the BPC of 1.54 reported in \cite{mikolov2012subword} with Multiplicative RNN (MRNN). 
%The validation curve, displayed in Figure~\ref{fig:4architec}(a),
%further shows the gap between
%\textit{td} and the other three architectures.
%Even though \textit{td}'s validation BPC is higher
%at the beginning of the training (possibly due to harder initial optimization),
%it outperforms all other architectures in the long run.
It is also interesting to note the 
improvement we obtain when switching from \textit{bu} to \textit{td}.  
The only difference between these two architectures 
lies in changing the direction of one connection (see Figure \ref{fig:depth_graph}(a)), 
which also increases
the recurrent depth. Such a fundamental difference is by no means
self-evident, 
but this result highlights the necessity of the concept of
recurrent depth.

\begin{figure}[!t]
\vspace{-10pt}
\centering
\minipage{0.42\textwidth}
    \includegraphics[width=\linewidth]{./figures/depth_graph.pdf}
\endminipage \hfill
\minipage{0.56\textwidth}%
    \includegraphics[width=\linewidth]{./figures/shallowness_graph.pdf}
\endminipage
%\minipage{0.33\textwidth}
%  \includegraphics[width=\linewidth]{ptb_valid_curve.pdf}
%\endminipage
\vspace{-5pt}
\caption{\small
\textbf{Left}: (a) The architectures for $sh$, $st$, $bu$ and $td$, with their
$(d_r, d_f)$ equal to $(1, 2)$, $(1, 3)$, $(1, 3)$ and $(2, 3)$, respectively.
The longest path in $td$ are colored in red.
(b) The 9 architectures denoted by their $(d_f, d_r)$ with 
 $d_r = 1, 2, 3$ and $d_f = 2, 3, 4$.
In both (a) and (b),
we only plot hidden states at two adjacent time steps and the connections between them (the period number is 1).
\textbf{Right}: (a) Various architectures that we consider 
in Section \ref{sec:diff_skip}.
From top to bottom are baseline $s=1$, and $s = 2$, $s = 3$. 
(b) Proposed architectures that we consider 
in Section \ref{sec:skip_nontrivial} where we take $k = 3$ as an example.
The shortest paths in (a) and (b) that correspond to the
recurrent skip coefficients are colored in blue.
}
\label{fig:depth_graph}
\vspace{-5pt}
\end{figure}


\begin{table}[t]
\vspace{-0pt}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|c|c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c}
\hline
\hline
%\abovespace\belowspace
Dataset&Models\char92 Archs &\textit{sh} & \textit{st} & \textit{bu} & \textit{td} \\
\hline
%\abovespace
PennTreebank&$\tanh$ RNN& 1.54& 1.59& 1.54& \textbf{1.49}\\
\hline
&$\tanh$ RNN-small & 1.80 & 1.82 & 1.80 & \textbf{1.77} \\
text8&$\tanh$ RNN-large & 1.69 & 1.67 & 1.64 & \textbf{1.59} \\
%\belowspace
%\abovespace
&LSTM-small&1.65 & 1.66 & 1.65 & \textbf{1.63} \\
&LSTM-large&1.52 & 1.53 & 1.52 & \textbf{1.49} \\
%\belowspace
\hline
\end{tabular}
\hspace{10pt}
\begin{tabular}{c|@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c}
\hline
\hline
$d_f$\char92$d_r$&$d_r$ = 1 & $d_r$ = 2 & $d_r$ = 3\\
\hline
 $d_f$ = 2 & 1.88 & 1.86 & 1.86\\
 $d_f$ = 3 & 1.86 & \textbf{1.84} & 1.86\\
 $d_f$ = 4 & 1.85 & 1.86 & 1.88\\
\hline
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{\small \textbf{Left}: Test BPCs of \textit{sh}, \textit{st}, \textit{bu}, \textit{td} for $\tanh$ RNNs
and LSTMs. \textbf{Right}: Test BPCs of $\tanh$ RNNs with recurrent depth $d_r = 1, 2, 3$ and feedforward depth
$d_f = 2, 3, 4$ respectively.}
\label{tb:butd}
\vspace{-25pt}
\end{table}

%\begin{figure}[t]
%\vspace{-8pt}
%\includegraphics[width=\columnwidth]{./figures/depth_graph.pdf}
%\vspace{-22pt}
%\caption{(a) the architectures for $sh$, $st$, $bu$ and $td$, with their
%$(d_r, d_f)$ equal to $(1, 2)$, $(1, 3)$, $(1, 3)$ and $(2, 3)$, respectively.
%The longest path in $td$ are colored in red.
%(b) The 9 architectures denoted by their $(d_f, d_r)$ with 
% $d_r = 1, 2, 3$ and $d_f = 2, 3, 4$.
%We only plot the hidden states within 1 time step (which also have a period of 1) in
%both (a) and (b).}
%\label{fig:depth_graph}
%\vspace{-10pt}
%\end{figure}

%\begin{figure}[t]
%\vspace{-5pt}
%\centering
%\includegraphics[width=170pt]{./figures/butd_main.pdf}
%\vspace{-20pt}
%\caption{Validation curves of $sh$, $st$, $bu$ and $td$ on text8 dataset.}
%\label{fig:4architec}
%\vspace{-10pt}
%\end{figure}


%\begin{figure*}[t]
%\vspace{-5pt}
%\includegraphics[width=\textwidth]{./figures/depth_newcurve.pdf}
%\vspace{-30pt}
%\caption{Validation curves for architectures with different $d_r$ and $d_f$.
%(a) Fix $d_f = 2$, change $d_r$ from $1$ to $3$.
%(b) Fix $d_f = 3$, change $d_r$ from $1$ to $3$.
%(c) Fix $d_r = 1$, change $d_r$ from $2$ to $4$.
%(d) Fix $d_r = 2$, change $d_r$ from $2$ to $4$.}
%\label{fig:depth_curve}
%\vspace{-10pt}
%\end{figure*}
\ \ \\
\vspace{-5pt}
\subsection{Comparing Depths}
\vspace{-5pt}
\label{sec:full}
From the previous experiment,
we found some evidence that with larger recurrent depth, the performance might improve. To further investigate various implications of depths, 
we carry out a systematic analysis for
both recurrent depth $d_r$ and feedforward depth $d_f$ on text8 and sequential MNIST datasets.
We build $9$ models in total with
$d_r = 1, 2, 3$ and $d_f = 2, 3, 4$, respectively (as shown in Figure \ref{fig:depth_graph}(b)).
%The way we are increasing the depth is by simply stacking layers
%vertically or horizontally, as shown in Fig. \ref{fig:depth_graph} (b).
We ensure that all the models have roughly the same number of parameters 
(e.g., the model with $d_r=1$ and $d_f=2$ has a hidden-layer size of $360$).

%\begin{table}[h]
%\vspace{-10pt}
%\caption{Test BPCs of 9 architectures with different $d_r$, $d_f$, $\tanh$}
%\label{tb:3x3}
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{c|@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c}
%\hline
%\hline
%%\abovespace\belowspace
%test BPC, text8&$d_r = 1$ & $d_r = 2$ & $d_r = 3$\\
%\hline
% $d_f = 2$ & $1.88$ & $1.84$ & $\mathbf{1.83}$\\
% $d_f = 3$ & $1.86$ & $1.84$ & $1.85$\\
% $d_f = 4$ & $1.94$ & $1.89$ & $1.88$\\
%\hline
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vspace{-5pt}
%\end{table}

Table \ref{tb:butd}, right panel, displays results 
on the text8 dataset. We observed that when fixing feedforward
depth $d_f = 2, 3$ (or fixing recurrent depth $d_r = 1, 2$),
increasing recurrent depth $d_r$ from 
$1$ to $2$ (or increasing feedforward depth $d_f$ from $2$ to $3$) does improve the model performance.
The best test BPC is achieved by the architecture
with $d_f =3, d_r = 2$. 
%Not sure how to interprete this 
This suggests that reasonably increasing $d_r$ and $d_f$
can aid in better capturing the over-time
nonlinearity of the input sequence. %, which is consistent with our theory of $d_r$. 
However, for too large $d_r$ (or $d_f$) like $d_r=3$ or $d_f = 4$, increasing $d_f$ (or $d_r$) only
hurts models performance. 
This can potentially be attributed to the optimization issues when modelling large input-to-output 
dependencies (see Appendix \ref{sec:full_com} for more details).
%Table \ref{tb:butd}, right panel, displays results 
%on the text8 dataset. We observed that for a fixed feedforward depth $d_f$,
%increasing the recurrent depth $d_r$ does improve the model performance,
%and the best test BPC is achieved by the architecture
%with $d_f = 2$ and $d_r = 3$. 
%%Not sure how to interprete this 
%This suggests that the increase of $d_r$
%can aid in better capturing the over-time
%nonlinearity of the input sequence. %, which is consistent with our theory of $d_r$. 
%However, for a fixed $d_r$, increasing $d_f$ only helps
%when $d_r = 1$. For a recurrent  
%depth of $d_r = 3$, increasing $d_f$ only hurts models performance. 
%This can potentially be attributed to the optimization issues when modelling large input-to-output 
%dependencies (see Appendix \ref{sec:full_com} for more details).
%\textcolor{red}{TODO:Do we need compare our results to SOTA on text8?}
%is possibly due to the fact that the increase of $d_r$ also
%brings potential optimization problems which makes the model
%We also tried another 
With sequential MNIST dataset, we next examined the effects of $d_f$ and $d_r$ 
when modelling long term dependencies (more in Appendix \ref{sec:full_com}).
In particular, we observed that 
increasing $d_f$ does not bring any improvement to the model performance,
and increasing $d_r$ might even be detrimental for training. 
%This is also 
%consistent with our theory: 
Indeed, it appears that $d_f$ only captures the local nonlinearity
and has less effect on the long term prediction.
This result seems to contradict previous claims~\citep{hermans2013training} that stacked RNNs ($d_f > 1$, $d_r=1$)
could capture information in different time scales and would thus
be more capable of dealing with
learning long-term dependencies. On the other hand, 
a large $d_r$ indicates multiple transformations per time step, resulting in greater
gradient vanishing/exploding issues~\cite{pascanu2013construct}, which suggests
that $d_r$ should be neither too small nor too large.
%Increasing $d_r$ and $d_f$ within a reasonable range
%may yield better performance, while excessive increase might
%result in serious optimization issues. For long term dependency tasks, $d_r$ and $d_f$ might not be the correct measures to consider.
%The test table shows the result on RNN with $\tanh$. One can observe
%that as the recurrent depth increases, the model benefits from its
%increasing nonlinearities, and yields better predictions.
%\textcolor{red}{TODO:Finish the section.} 

\vspace{-5pt}
\subsection{Recurrent Skip Coefficients}
\vspace{-5pt}
\label{sec:diff_skip}
To investigate whether increasing a recurrent skip coefficient $s$ improves
model performance on long term dependency tasks, we compare models with
increasing $s$ on the adding problem, the copying memory problem and the sequential MNIST
problem (without/with permutation, denoted as MNIST and $p$MNIST). 
Our baseline model is the shallow architecture proposed in \cite{le2015simple}. To increase
the recurrent skip coefficient~$s$, we add
connections from time step $t$ to 
time step $t+k$ for some fixed integer $k$, shown in Figure \ref{fig:depth_graph}(a), right panel.
By using this specific construction, the recurrent skip
coefficient increases from 1 (i.e., baseline) to $k$ and the new model 
with extra connection has
$2$ hidden matrices (one from $t$ to $t+1$ and
the other from $t$ to $t+k$). 
%For each experiment we ensure that models have roughly the same number of 
%parameters.

For the adding problem, we follow the same setting as in \cite{arjovsky2015unitary}.
We evaluate the baseline LSTM with 128 hidden units and an LSTM with $s = 30$
and 90 hidden units (roughly the same number of parameters as the baseline). 
The results are quite encouraging: as suggested in \cite{arjovsky2015unitary} baseline
LSTM works well for input sequence lengths $T = 100, 200, 400$ but fails when
$T= 750$. On the other hand, we observe that the LSTM with  $s = 30$ learns
perfectly when $T = 750$, and even if we increase
$T$ to 1000, LSTM with $s = 30$ still works well and the loss reaches to zero.  

For the copying memory problem, we use a single layer RNN
with 724 hidden units as our basic model, and 512 hidden units with skip connections.
So they have roughly the same number of parameters.
Models with a higher recurrent skip coefficient outperform those without skip 
connections by a large margin. 
When $T=200$, test set cross entropy (CE) of a basic model only yields 0.2409, 
but with $s=40$ it is able to reach a test set cross entropy of 0.0975. %, only around one third of its conterpart. 
When $T=300$, a model with $s=30$ yields a test set CE of 0.1328,
while its baseline could only reach 0.2025.
We varied the sequence length ($T$) and recurrent skip coefficient
($s$) in a wide range (where  $T$ varies from 100 up to 300, and $s$ from 10
up to 50), and found that this kind of improvement persists. 


For the sequential MNIST problem, the hidden-layer size of the baseline model
is set to $90$ and models with $s>1$ have hidden-layer sizes of~$64$.
\begin{table}[!t]
\vspace{-10pt}
\label{tb:diff_skip}
\centering
\small
\begin{tabular}{c@{\hspace{2pt}}|@{\hspace{4pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c}
\hline
\hline
%\abovespace\belowspace
s$\tanh$ & s = 1 & s = 5 & s = 9 & s = 13 & s = 21\\
  MNIST&34.9 &46.9 &74.9 &85.4  & \textbf{87.8}\\
\hline
   &s = 1 & s = 3 & s = 5 & s = 7 &s = 9\\
 $p$MNIST &49.8 &79.1 &84.3 &\textbf{88.9}  &88.0\\
\hline
\end{tabular}
\quad
\begin{tabular}{c@{\hspace{2pt}}|@{\hspace{4pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c@{\hspace{6pt}}c}
\hline
\hline
LSTM & s = 1 & s = 3 & s = 5 & s = 7 & s = 9\\
  MNIST&56.2 &\textbf{87.2} &86.4 &86.4  & 84.8\\
\hline
  & s = 1 & s = 3 & s = 4 & s = 5 &s = 6\\
 $p$MNIST  &28.5 &25.0 &60.8 &62.2  &\textbf{65.9}\\
\hline
\end{tabular}
\\
\vspace{5pt}
\begin{tabular}{c|ccc}
\hline
\hline
%\abovespace\belowspace
Model & MNIST  & $p$MNIST\\
\hline
iRNN\cite{le2015simple} &  97.0& $\approx$82.0\\
uRNN\cite{arjovsky2015unitary}& 95.1&  91.4 \\
LSTM\cite{arjovsky2015unitary} &\textbf{98.2}& 88.0\\
RNN($\tanh$)\cite{le2015simple}& $\approx$35.0& $\approx$35.0\\
\hline
s$\tanh$(s = 21, 11) &98.1& \textbf{94.0}\\
\hline
\end{tabular}
\hspace{7pt}
\begin{tabular}{r@{\hspace{5pt}}|@{\hspace{5pt}}c@{\hspace{8pt}}c@{\hspace{8pt}}c@{\hspace{8pt}}c@{\hspace{8pt}}c}
\hline
\hline
%\abovespace\belowspace
Architecture, s\hspace{4pt} &(1), 1 & (2), 1& (3), $\frac{k}{2}$& (4), $k$  \\
\hline     
MNIST\hspace{2pt} k = 17 & 39.5& 39.4  & 54.2 & \textbf{77.8} \\
 k = 21 & 39.5& 39.9  &69.6 &\textbf{71.8} \\
\hline
$p$MNIST\hspace{5pt} k = 5 & 55.5& 66.6  & 74.7 & \textbf{81.2}\\
\hspace{12pt}k = 9 & 55.5& 71.1  &78.6 &\textbf{86.9}  \\
\hline
\end{tabular}

\hspace{10pt}
\vspace{0pt}
\caption{\small Results for MNIST/$p$MNIST.
\textbf{Top-left}: Test accuracies with different $s$ for $\tanh$ RNN.
\textbf{Top-right}: Test accuracies with different $s$ for LSTM.
\textbf{Bottom-left}: Compared to previous results.
\textbf{Bottom-right}: Test accuracies for architectures (1), (2), (3)
and (4) for  $\tanh$ RNN.}
\label{tb:mnist}
\vspace{-25pt}
\end{table}
%\begin{figure}[t]
%\includegraphics[width=\columnwidth]{./figures/shallowness_graph.pdf}
%\vspace{-20pt}
%\caption{(a) Various architectures that we consider 
%in Section \ref{sec:diff_skip}.
%From top to bottom are baseline $s=1$, and $s = 2$, $s = 3$. 
%(b) Proposed architectures that we consider 
%in Section \ref{sec:skip_nontrivial} where we take $k = 3$ as an example.
%The shortest paths in (a) and (b) that correspond to the
%recurrent skip coefficients are colored in blue.}
%\label{fig:diff_skip}
%\vspace{-10pt}
%\end{figure}
The results in Table~\ref{tb:mnist}, top-left panel, show that $\tanh$ RNNs with recurrent 
skip coefficient $s$ larger than $1$ could improve the model performance dramatically.
Within a reasonable range of $s$, test accuracy increases quickly as $s$ becomes
larger. We note that our model is the first $\tanh$ RNN model
that achieves good performance on this task,
even improving upon the method proposed in~\cite{le2015simple}.
% with less parameters
%on $p$MNIST. 
In addition, we also formally compare with the previous results reported in 
\cite{le2015simple, arjovsky2015unitary}, where our model (referred to as s$\tanh$)
has a hidden-layer size of $95$, which is about the same number of parameters as in the $\tanh$ model of
\cite{arjovsky2015unitary}.
Table \ref{tb:mnist}, bottom-left panel, shows 
that our simple architecture
improves upon the $u$RNN by $2.6\%$ on $p$MNIST,
and achieves almost the same performance as LSTM on the MNIST dataset with only $25\%$ number of parameters  
~\cite{arjovsky2015unitary}.
Note that obtaining good performance on sequential MNIST requires a larger $s$ than that for
$p$MNIST (see Appendix~\ref{sec:full_com} for more details).
LSTMs also showed performance boost and much faster
convergence speed when using larger $s$, as displayed in Table~\ref{tb:mnist}, top-right panel.
LSTM with $s=3$ already
performs quite well and increasing $s$ did not result in any significant improvement,
while in $p$MNIST, the performance gradually improves  as $s$ increases
from $4$ to $6$. We also observed that the LSTM network performed worse on permuted MNIST
compared to a $\tanh$ RNN. Similar result was also reported in~\cite{le2015simple}.




% We provide an hypothesis for why this happens in Appendix \ref{sec:full_com}.


%\begin{figure*}[t]
%\includegraphics[width=\textwidth]{./figures/mnist.pdf}
%\vspace{-20pt}
%\caption{Test accuracies of $\tanh$ RNN and LSTM  
%with different recurrent skip coefficients (numbers in the legend) on MNIST and $p$MNIST datasets.}
%\label{fig:mnist_curve}
%\vspace{-10pt}
%\end{figure*}


%\begin{table}[h]
%\vspace{-15pt}
%\caption{Test accuracies on sequential MNIST and pMNIST tasks}
%\label{tb:sota}
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{c|ccc}
%\hline
%\hline
%%\abovespace\belowspace
%test acc $(\%)$ & MNIST  & $p$MNIST\\
%\hline
%$i$RNN\cite{le2015simple} &  $97.0$& $\approx82.0$\\
%$u$RNN\cite{arjovsky2015unitary}& $95.1$&  $91.4$ \\
%LSTM\cite{arjovsky2015unitary} &$\mathbf{98.2}$& $88.0$\\
%tanh\cite{le2015simple}& $\approx35.0$& $\approx35.0$\\
%\hline
%$s$tanh($s = 21, 11$) &$98.1$& $\mathbf{94.0}$\\
%\hline
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vspace{-5pt}
%\end{table}

%\begin{table}[!t]
%\vspace{-10pt}
%\label{tb:diff_skip}
%\centering
%\small
%\begin{tabular}{r@{\hspace{5pt}}|@{\hspace{5pt}}c@{\hspace{8pt}}c@{\hspace{8pt}}c@{\hspace{8pt}}c@{\hspace{8pt}}c}
%\hline
%\hline
%%\abovespace\belowspace
%Architecture, s\hspace{4pt} &(1), $1$ & (2), $1$& (3), $\frac{k}{2}$& (4), $k$  \\
%\hline     
%MNIST\hspace{2pt} $k = 17$ & $39.5$& $39.4$  & $54.2$ & $\mathbf{77.8}$ \\
% $k = 21$ & $39.5$& $39.9$  &$69.6$ &$\mathbf{71.8}$  \\
%\hline
%$p$MNIST\hspace{5pt} $k = 5$ & $55.5$& $66.6$  & $74.7$ & $\mathbf{81.2}$ \\
%\hspace{13pt}$k = 9$ & $55.5$& $71.1$  &$78.6$ &$\mathbf{86.9}$  \\
%\hline
%\end{tabular}
%\vspace{5pt}
%\caption{\small Test accuracies for architectures (1), (2), (3)
%and (4) for  $\tanh$ RNN on MNIST/$p$MNIST}
%\label{tb:mnist}
%\vspace{-10pt}
%\end{table}
\vspace{-5pt}
\subsection{Recurrent Skip Coefficients vs. Skip Connections}
\vspace{-5pt}
\label{sec:skip_nontrivial}
We also investigated whether the recurrent skip coefficient can suggest something more than simply adding skip connections. We design 4 specific 
architectures shown in Figure \ref{fig:depth_graph}(b), right panel.
(1) is the baseline model with a 2-layer stacked architecture,
while the other three models add extra skip connections in different ways.
Note that \textbf{these extra skip connections
all cross the same time length $k$}.
In particular, (2) and (3) share quite similar architectures.
However, ways in which the skip connections are allocated 
makes big differences on their recurrent skip coefficients: (2) has $s = 1$,
(3) has $s = \frac{k}{2}$ and (4) has $s = k$. 
Therefore, even though (2), (3) and (4) all add extra skip connections, the fact that their recurrent skip coefficients are different might result in different performance.

We evaluated these architectures on the sequential MNIST and
$p$MNIST datasets. The results show that differences in~$s$
indeed cause big performance gaps regardless of the fact that they
all have skip connections (see Table~\ref{tb:mnist}, bottom-right panel).
Given the same $k$, the model with a larger $s$ performs better. 
In particular, model~(3) is better than model~(2) even though they only differ in the direction of the skip connections.
It is interesting to see that for MNIST (unpermuted), the extra skip connection
in model (2) (which does not really increase the recurrent skip coefficient)
brings almost no benefits, as model (2) and model (1) have 
almost the same results.
This observation
highlights the following point: when addressing
the long term dependency problems using skip connections,
instead of only considering the time intervals crossed by
the skip connection, one should also consider the model's
recurrent skip coefficient, which can serve as a guide for introducing more powerful skip connections.

\vspace{-8pt}
\section{Conclusion}
\vspace{-7pt}
In this paper, we first introduced a general formulation of RNN architectures, which provides a solid framework for the architectural complexity analysis. We then proposed three architectural complexity measures: recurrent depth, feedforward depth, and recurrent skip coefficients capturing both short term and long term properties of RNNs.
We also found empirical evidences that 
increasing recurrent depth and feedforward depth might yield performance improvements, increasing feedforward depth might not help on long
term dependency tasks, while increasing the recurrent skip coefficient
can largely improve performance on long term dependency tasks. 
These measures and results can provide guidance for the design of new 
recurrent architectures for particular learning tasks.
%Future work could involve more comprehensive studies (e.g., providing analysis on more datasets, using different architectures with various transition functions) to investigate the effectiveness of the proposed measures. 
\vspace{-5pt}
\section*{Acknowledgments}
\vspace{-10pt}
The authors acknowledge the following agencies for funding and support: NSERC, Canada Research Chairs, CIFAR, Calcul Quebec, Compute Canada, Samsung,
ONR Grant N000141310721, ONR Grant N000141512791 and 
IARPA Raytheon BBN Contract No. D11PC20071. 
The authors thank the developers of Theano \cite{team2016theano} and Keras \cite{chollet2015}, and also thank Nicolas Ballas,
Tim Cooijmans, Ryan Lowe, Mohammad Pezeshki, Roger Grosse and Alex Schwing for their insightful comments.
\newpage
{\small 
\bibliography{1recdepth}
\bibliographystyle{unsrt}
}

